Varianceflow: High-Quality and Controllable Text-to-Speech using Variance Information via Normalizing Flow

There are two types of methods for non-autoregressive text-to-speech models to learn the one-to-many relationship between text and speech effectively. The first one is to use an advanced generative framework such as normalizing flow (NF). The second one is to use variance information such as pitch or energy together when generating speech. For the second type, it is also possible to control the variance factors by adjusting the variance values provided to a model. In this paper, we propose a novel model called VarianceFlow combining the advantages of the two types. By modeling the variance with NF, VarianceFlow predicts the variance information more precisely with improved speech quality. Also, the objective function of NF makes the model use the variance information and the text in a disentangled manner resulting in more precise variance control. In experiments, VarianceFlow shows superior performance over other state-of-the-art TTS models both in terms of speech quality and controllability.

==> 3_relatedwork.tex <==
\section{Related Work}
\textcolor{red}{Is this too much overllaped with Introduction?}
Although early autoregressive (AR) TTS models such as Tacotron 2 or Transformer-TTS \cite{Wang2017, li2019neural} show great speech quality, autoregressive modeling has several inherent shortcomings.
%
First, speech generation can not be parallelized due to its sequential generation property.
%
Second, the errors such as mispronouncing or word skipping gets more frequent when input text is longer, which is inevitable due to the error propagation property inherent in AR models.
Therefore, several non-AR TTS models have been proposed and they have mainly focused on two problems: (1) how to find alignment between text and speech; (2) how to train a model to learn the complex speech distribution.
In this paper, we suppose that the alignment problem can be easily solved by utilizing ground-truth durations of phonemes, and we focus on the second problem and describe how we solve it.

\subsection{Using an advanced generative model}
The early non-AR TTS models \cite{NEURIPS2019_f63f65b5, Peng2020nonautoregressive} had difficulty in learning the complex speech distribution using the mean-square error (MSE) loss since it assumes that the target distribution follows gaussian distribution.
Therefore, they used autoregressive models as teacher models, but their speech quality were still inferior to the AR TTS models.
Recently, non-AR TTS models have been shown better speech quality compared to the AR TTS models by adopting advanced generative models that do not assume any pre-defined distribution form.
For example, Glow-TTS \cite{NEURIPS2020_5c3b99e8} uses normalizing flow to decode the aligned text representations and Diff-TTS \cite{jeong21_interspeech} uses denosing deffusion probabilistic model as a decoder and shows the state-of-the-art speech quality.
Also, GANSpeech \cite{yang21e_interspeech} shows that using additional adversarial loss in addition to the MSE loss is effective to improve its speech quality.

\subsection{Using an additional varaince information}
Instead of using advanced generative models, FastSpeech 2 \cite{ren2021fastspeech} utilizes additional variance information such as pitch and energy.
Added to the text representations before passed to the decoder, the variance information simplifies the complexity of speech distribution, so it significantly improves the convergence speed and speech quality.
The additional advantage of this method is the fact that it is possible to control the variance factors by manipulating the predicted variance values.
  
At inference, since it is impossible to provide the ground-truth variance information, pitch and energy values that are predicted by variance predictors are used in FastSpeech 2.
However, there is still a problem that, although it is important to predict the variance values well to get natural speech, predicting pitch or energy from a text is also a difficult task having one-to-many problem.
For this, FastSpeech 2 trains the pitch predictor with continuous wavelet transformed pitch spectrogram instead of raw pitch values.
Also, FastPitch, which uses pitch information similar to FastSpeech 2, uses phoneme-averaged pitch values to ease the difficulty of learning the complex pitch distribtuion.
\footnote{Many unofficial FastSpeech 2 implementations also report that using phoneme-averaged pitch values show better speech quality.  
  
https://github.com/espnet/espnet  
  
https://github.com/TensorSpeech/TensorFlowTTS  
  
https://github.com/ming024/FastSpeech2}

==> tables/control_mos.tex <==
\begin{table*}[t]
    \caption{Experimental results. The MOS-ID and MOS-OOD are written with 95\% confidence intervals. The number in parentheses represents the number of parameters of BVAE-TTS that are used at inference.}
    \vspace{0.5cm}
	\centering
	\begin{tabular}{ l | c c c c c c c }
		\toprule
		\multirow{3}{2.3em}{Model} & \multicolumn{7}{c}{\textbf{Pitch Shift Scale} ($\lambda$)}\\
		& -8 & -6 & -4 & 0 & +4 & +6 & +8\\
		& (63\%) & (71\%) & (79\%) & (100\%) & (126\%) & (141\%) & (159\%)\\
		\midrule
		GT Audio & - & - & - & 4.55 & - & - & - \\
		GT Mel-spectrogram & - & - & - & 4.41 & - & - & - \\
		\midrule
		FastSpeech2-phone & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85\\
		FastSpeech2-frame & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85\\
		VarianceFlow-phone & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85\\
		VarianceFlow-frame & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85\\
		VarianceFlow-frame-reversed & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85 & 3.85\\
		\bottomrule
	\end{tabular}
	\label{tab: control_mos}
\end{table*}
\vspace{0.5cm}
